Tensorized Pauli decomposition algorithm

This paper introduces a novel general-purpose algorithm for Pauli decomposition that employs matrix slicing and addition rather than expensive matrix multiplication, significantly accelerating the decomposition of multi-qubit matrices. In a detailed complexity analysis, we show that the algorithm admits the best known worst-case scaling and more favorable runtimes for many practical examples. Numerical experiments are provided to validate the asymptotic speed-up already for small instance sizes, underscoring the algorithm's potential significance in the realm of quantum computing and quantum chemistry simulations.

==> specs.tex <==
\begin{tabular}{| r l |}\hline
	Processor & Intel(R) Core(TM) i5-1035G1 CPU @ 1.00GHz   1.20 GHz \\\hline
	RAM & 8,00 GB \\
	OS & Windows 10 Pro (22H2) \\
	python & 3.10.4 \\
	numpy & 1.25.2 \\
	scipy & 1.11.1 \\
	qiskit & 1.0.2 \\
	pennylane & 0.31.1
    \hline
\end{tabular}

